Asymmetric Coded Caching for Multi-Antenna Location-Dependent Content Delivery

Efficient usage of in-device storage and computation capabilities are key solutions to support data-intensive applications such as immersive digital experiences. This paper proposes a location-dependent multi-antenna coded caching -based content delivery scheme tailored specifically for wireless immersive viewing applications. First, a novel memory allocation process incentivizes the content relevant to the identified wireless bottleneck areas. This enables a trade-off between local and global caching gains and results in unequal fractions of location-dependent multimedia content cached by each user. Then, a novel packet generation process is carried out during the subsequent delivery phase, given the asymmetric cache placement. During this phase, the number of packets transmitted to each user is the same, while the sizes of the packets are proportional to the corresponding location-dependent cache ratios. In this regard, each user is served with location-specific content using joint multicast beamforming and a multi-rate modulation scheme that simultaneously benefits from global caching and spatial multiplexing gains. Numerical experiments and mathematical analysis demonstrate significant performance gains compared to the state-of-the-art.

==> Figs/Data/Figrate.tex <==
States	rates	Memory
1	3	0.25
2	2	0.50
3	1	0.75
4	2	0.50
5	3	0.25


==> SimResults.tex <==
\section{Simulation Results}
\label{sec:Simulations}
We use numerical simulations to evaluate the performance of the proposed location-dependent scheme. We consider a bounded $5 \times 5 \ [\text{m}^2]$ room divided into $S = 121$ states, where a transmitter with $L=2$ antennas is located in the middle of the room on the ceiling at $3$ [m] height. The channel at state $s \in \mathcal{S}$ is modelled as $\Bh({s}) \sim \mathbb{CN}(\mathbf{0}, {\sigma_s}{d^{-\eta}_{s}}\BI)$, where $d_s$ is the distance between the center of the state $s$ and the transmitter, $\eta = 3$ is the pass-loss exponent and $\sigma_s$ is the shadowing effect. To reflect the shadowing effect, we assume $B$ states (out of $S$ states) are highly attenuated (e.g., located behind obstacles like walls, etc. see Fig.~\ref{fig:system-model}). We assume a simple binary attenuation model for $\sigma_s$, where $\sigma_s=1$ for non-attenuated states and $\sigma_s=\beta$ for attenuated ones. We assume the transmit power is set such that the received \ac{SNR} at the non-attenuated states at the room borders is equal to  $P_T$ [dB]. For a user $k$ located in state $s$ during the delivery phase, we assume $\Bh_k = \Bh(s)$. At each time-slot, users $k=1,\ldots, K$ are placed in any state $s=1,\ldots, S$ with uniform probability. For comparison, we use both the total transmission time to serve all the users $T_T$ and symmetric rate, defined as $\frac{K}{T_T}$, averaged over all channel realizations. In all the simulations, we use optimized weighted max-min beamformers obtained by solving~\eqref{opt:nonconvex_WMMF}.

%We use numerical simulations to evaluate the performance of the proposed location-dependent scheme. We consider a bounded $5 \times 5 \ [\text{m}^2]$ room divided into $S = 121$ states, where a transmitter with $L=2$ antennas is located in the middle of the room on the ceiling at $3$ [m] height. The channel at state $s \in \mathcal{S}$ is modelled as $\Bh_{s} \sim \mathbb{CN}(\mathbf{0}, {\sigma_s}{d^{-\eta}_{s}}\BI)$, where $d_s$ is the distance between the center of the state $s$ at the ground and the transmitter, $\eta = 3$ is the pass-loss exponent and $\sigma_s$ is the shadowing effect. To reflect the shadowing effect, we assume $B$ states (out of $S$ states) are highly attenuated (e.g., located behind obstacles like walls, etc. see Fig.~\ref{fig:system-model}). We assume a simple binary attenuation model for $\sigma_s$, where $\sigma_s=1$ for non-attenuated states and $\sigma_s=\beta$ for attenuated ones. We assume the transmitter is able to provide $P_T$ power at the non-attenuated cell-edge states and the noise floor is set to be $N_0 = 1$. For a user $k$ located in state $s$ during the delivery phase, we assume $\Bh_k = \Bh(s)$. At each time-slot, users $k=1,\ldots, K$ are placed in any state $s=1,\ldots, S$ with uniform probability. For comparison, we use both the total required time to serve all the users $T_T$ and symmetric rate, defined as $\frac{K}{T_T}$, averaged over all channel realizations. In all the simulations, we use optimized weighted max-min beamformers obtained by solving~\eqref{opt:nonconvex_WMMF}.

% The proposed scheme is compared with three benchmark methods. \textbf{Unicast uniform}  \textbf{unicast non-uniform} represents location-dependent cache placement followed by unicast delivery, and \textbf{MN-uniform} refers to uniform cache allocation and conventional \ac{CC} delivery of~\cite{tolli2017multi}. 

We consider eight benchmark schemes, as the following
\begin{itemize}
    \item \textbf{\textit{Uni}}: Uniform cache allocation followed by unicast delivery using spatial multiplexing and local caching gain only (i.e., serving $L$ users during each transmission).
    \item \textbf{\textit{Unim}}: Location-dependent cache placement (for $\phi \gg 1$) followed by unicast delivery.
    \item \textbf{\textit{Unimm}}: Location-dependent cache placement (for $\phi = \frac{L}{K}$) followed by unicast delivery.
    \item \textbf{\textit{MNm}}: The proposed cached placement and delivery scheme (for $\phi \gg 1$) without \emph{phantom-user} scheme.
    \item \textbf{\textit{MNmp}}: The proposed cached placement and delivery scheme (for $\phi \gg 1$) complemented by \emph{phantom-user} scheme.
    \item \textbf{\textit{MNmm}}: The proposed cached placement and delivery scheme (for $\phi = \frac{L}{K}$) without \emph{phantom-user} scheme.
    \item \textbf{\textit{MNmmp}}: The proposed cached placement and delivery scheme (for $\phi = \frac{L}{K}$) complemented by \emph{phantom-user} scheme.
    \item \textbf{\textit{MN}}: Uniform cache allocation and conventional \ac{CC} delivery of~\cite{tolli2017multi}.
\end{itemize}

\begin{figure*}[ht]
\begin{minipage}[c]{0.49\textwidth} 
\centering 
\setlength\abovecaptionskip{-0.25\baselineskip}
\includegraphics[width=1\columnwidth,keepaspectratio]{Figs/blockage_rate.eps}
\caption{Rate versus the number of attenuated states ($B$).}
\label{fig:sim_B_rate}
\end{minipage}
\hspace{2mm}
\begin{minipage}[c]{0.49\textwidth}
\centering 
\setlength\abovecaptionskip{-0.25\baselineskip}
\includegraphics[width=1\columnwidth,keepaspectratio]{Figs/blockage_time.eps}
\caption{Delivery time (log-scale) versus the number of attenuated states ($B$).}
\label{fig:sim_B_time}
\end{minipage}
\end{figure*} 

% \begin{figure}
%     \centering 
%     \includegraphics[width=0.8\columnwidth,keepaspectratio]{figs/simulation/blockage.eps}
%     \caption{Symmetric rate versus different number of attenuated states ($B$).}
%     \label{fig:simu_B}
% \end{figure}

Figures~\ref{fig:sim_B_rate}, compares the average symmetric rate of different benchmarks for a different number of attenuated states ($B$). As illustrated, when there is no attenuated state, the traditional caching scheme of \cite{tolli2017multi} outperforms other methods. This is because in the proposed schemes, we sacrifice the global caching gain, i.e., $t = \frac{KM}{S}$, for higher local caching gain, i.e., $m_i$, which results in a higher transmission rate ($R^{\textbf{sym}}_{\text{WMM}}$) compared to \cite{tolli2017multi}. Now, comparing the symmetric rate of \cite{tolli2017multi} with the proposed scheme $\frac{R^{\text{sym}}_{\text{WMM}}}{R^{\text{sym}}_{\text{MM}}} = \frac{(\hat{t}+L)R_{\text{WMM}}}{(t+L)R_{\text{MM}}}$, we can see that when different states have almost the same channel conditions, the performance loss due to the DoF decrements (i.e., $\frac{\hat{t}+L}{t+L}$) is more than the rate improvement (i.e., $\frac{R_{\text{WMM}}}{R_{\text{MM}}}$). However, when the number of blocked states grows, the uniform cache placement schemes "\emph{MN}" and "\emph{Uni}" perform poorly compared to the other memory-loading-based approaches. This is because the probability of finding a user in an attenuated state grows much more prominent with the number of attenuated states. Hence, likely there exist an ill-conditioned user in each transmission, limiting the transmission rate. On the other hand, the multicasting based memory-loading scheme of "\emph{MNmmp}" outperforms the rest for a limited number of attenuated states. This is because for $\phi = \frac{L}{K}$, the proposed memory loading in~\eqref{cache-allocation_dif_conv} allocates the same amount of memory $m(s)$ for those states with almost the same expected rates $r(s)$. As a result, the minimum achievable cache ratio is boosted in this case. However, this results in less gain for the phantom-user scheme as the cache ratio diversity decreases in this case. Therefore, as the number of attenuated states grows, the minimum achievable cache ratio decreases (e.g., $\hat{t}$ falls below $1$ for $B \geq 20 \%$ in figure~\ref{fig:sim_B_rate}). At some point, the cache ratio boost is not as significant as the user diversity boost of the phantom-based scheme, which makes "\emph{MNmp}" a better option. Fig.~\ref{fig:sim_B_time}, makes the same comparison in the delivery time domain. As illustrated, even for a few attenuated states, the average delivery time of the uniform memory-loading schemes is highly worsened due to the near-far effect. However, this is not as obvious in the average symmetric rate plot.

\begin{figure*}[ht]
\begin{minipage}[c]{0.5\textwidth} 
\centering 
\setlength\abovecaptionskip{-0.25\baselineskip}
\includegraphics[width=1\columnwidth,keepaspectratio]{Figs/loss_rate.eps}
\caption{Symmetric rate versus attenuation level ($\beta$).}
\label{fig:sim_beta_rate}
\end{minipage}
\hspace{2mm}
\begin{minipage}[c]{0.5\textwidth}
\centering 
\setlength\abovecaptionskip{-0.25\baselineskip}
\includegraphics[width=1\columnwidth,keepaspectratio]{Figs/loss_time_log_scale.eps}
\caption{Delivery time (log-scale) versus attenuation level ($\beta$)}
\label{fig:sim_beta_time}
\end{minipage}
\end{figure*} 

Figures~\ref{fig:sim_beta_rate} and~\ref{fig:sim_beta_time} compare different methods for different attenuation levels $\beta$. As illustrated, the memory-loading-based schemes are hardly affected by increasing the attenuation level as they avoid wasting wireless resources on ill-conditioned states. Higher attenuation levels can quickly happen in higher frequencies or more concrete obstacles. However, it can be seen that at some point, the average achievable rate converges to some constant, which means that the achievable rate for some realization converges to zero. This is better illustrated in Fig.~\ref{fig:sim_beta_time}, which compares the average delivery time for different attenuation levels. As illustrated, the average delivery time grows unbounded for uniform memory loading schemes, whereas the rest are hardly affected. Thus, the conventional cc-based schemes (e.g., "\emph{MN}") can not be considered for time-critical applications such as immersive viewing due to extensive delivery time for ill-conditioned locations.

\begin{figure*}[ht]
\begin{minipage}[c]{0.5\textwidth} 
\centering 
\setlength\abovecaptionskip{-0.25\baselineskip}
\includegraphics[width=1\columnwidth,keepaspectratio]{Figs/power_rate.eps}
\caption{Symmetric rate versus received power ($P_T$).}
\label{fig:sim_power_rate}
\end{minipage}
\hspace{2mm}
\begin{minipage}[c]{0.5\textwidth}
\centering 
\setlength\abovecaptionskip{-0.25\baselineskip}
\includegraphics[width=1\columnwidth,keepaspectratio]{Figs/power_time_log_scale.eps}
\caption{Delivery time (log-scale) versus received power ($P_T$).}
\label{fig:sim_power_time}
\end{minipage}
\end{figure*} 

Figures~\ref{fig:sim_power_rate} and~\ref{fig:sim_power_time} compare different benchmarks for a different amount of received powers $P_T$. As illustrated, for lower received powers, the performance gap between the memory-loading based schemes and the uniform based schemes is more significant. In such scenarios, the achievable rate in different states is highly affected by the large and small scale effects. Thus, the memory-loading process results in significant wireless resource-saving. However, as the transmit power increases, the rate difference between different states become negligible, and the optimal memory loading converges to uniform memory-loading, i.e., "\emph{MN}". 

\begin{figure*}[ht]
\begin{minipage}[c]{0.5\textwidth} 
\centering 
\setlength\abovecaptionskip{-0.25\baselineskip}
\includegraphics[width=1\columnwidth,keepaspectratio]{Figs/memory_rate.eps}
\caption{Symmetric rate versus different memory size ($M/S$).}
\label{fig:sim_M_rate}
\end{minipage}
\hspace{2mm}
\begin{minipage}[c]{0.5\textwidth}
\centering 
\setlength\abovecaptionskip{-0.25\baselineskip}
\includegraphics[width=1\columnwidth,keepaspectratio]{Figs/memory_time_log_scale.eps}
\caption{Delivery time (log-scale) versus memory size ($M/S$).}
\label{fig:sim_M_time}
\end{minipage}
\end{figure*} 

In Figs.~\ref{fig:sim_M_rate} and~\ref{fig:sim_M_time} we have compared different methods based on different available memory at the users. It can be seen that the performance gap between the proposed method and the other schemes increases for higher available memory at the users. This is because with higher available memory, larger common coded caching gain $\hat{t}$ is achievable, which results in lower DoF loss compared to MN scheme, i.e., $\frac{\hat{t}+L}{t+L}$ approaches one for higher $M$. On the other hand, coded caching gain $\hat{t} = Km$ has another component, which is the number of users $K$. It is worth mentioning that due to the complex beamforming procedure for the MN-based schemes (such as the one proposed in this paper), we have considered a limited number of users in the network. However, by increasing the number of users in the network the common coded caching gain increases which results in higher performance gap compared to other methods as shown in Figs.~\ref{fig:sim_K_rate} and~\ref{fig:sim_K_time}.

\begin{figure*}[ht]
\begin{minipage}[c]{0.5\textwidth} 
\centering 
\setlength\abovecaptionskip{-0.25\baselineskip}
\includegraphics[width=1\columnwidth,keepaspectratio]{Figs/K_rate.eps}
\caption{Symmetric rate versus user count ($K$).}
\label{fig:sim_K_rate}
\end{minipage}
\hspace{2mm}
\begin{minipage}[c]{0.5\textwidth}
\centering 
\setlength\abovecaptionskip{-0.25\baselineskip}
\includegraphics[width=1\columnwidth,keepaspectratio]{Figs/K_time_log_scale.eps}
\caption{Average delivery time (log-scale) versus user count ($K$).}
\label{fig:sim_K_time}
\end{minipage}
\end{figure*} 

As illustrated in Figs.~\ref{fig:sim_K_rate} and~\ref{fig:sim_K_time}, the average delivery rate scales with the number of users for CC-based schemes due to a common cache ratio increment. However, as the worst user channel condition limits the uniform memory-loading based schemes, there is a rate drop in their achievable symmetric rate. Thus, on average, they perform worse for larger-sized networks. This is better illustrated in the average delivery time plot, which shows a considerable time increment for a larger number of users in uniform memory-loading schemes. On the other hand, phantom-based multiuser-memory-loading is less affected by the number of users, benefiting from local-caching and global caching gain efficiently. Finally, Fig.~\ref{fig:sim_cdf} plots the cumulative distribution function of the total delivery time for different realizations. As depicted, the MN scheme performs poorly for most cases, resulting in a high average delivery time. Note that for scenarios where users are located in relatively good conditioned states MN scheme provides much better delivery time and rate due to a higher common caching ratio, i.e., $t = \frac{KM}{S}$.

\begin{figure}
    \centering 
    \includegraphics[width=0.8\columnwidth,keepaspectratio]{Figs/blockage_time_cdf.eps}
    \caption{The cumulative distribution function (CDF) of total delivery time for $500$ realizations.}
    \label{fig:sim_cdf}
\end{figure}


==> beamforming.tex <==
\section{Weighted Max Min Beamforming}
\label{Sec:beamforming}

In example~\ref{exmp:coding-procedure}, we considered zero-forcing vectors $\Bv_{\CU}$ to nullify each message at ten users to serve each user interference-free. However, as argued in~\cite{tolli2017multi}, beamforming vectors $\{\Bv_{\CU}, \forall\CU \subseteq \hat{\CK}, \forall \hat{\CK} \subseteq \CK\}$ need not suppress the interference. Instead, they can be optimally designed to restrain it. Nevertheless, the symmetric rate considered in~\cite{tolli2017multi} is always limited to the users with bad channel conditions. Thus, Unlike~\cite{tolli2017multi}, which considers max-min-fairness to design precoders, we formulate the objective function as a weighted-max-min (WMM) problem. As a result, we can achieve higher rates by reducing the priority of ill-conditioned users.

Let us first review the delivery procedure to formulate the WMM problem. As described in section~\ref{sec:delivery}, at each time interval, the base station transmits $\binom{K}{\hat{t}+L}$ codewords $\Bx_{\hat{\CK}}$ in the \ac{TDMA} manner. Moreover, each transmitted codeword is comprised of $\binom{\hat{t}+L}{\hat{t}+1}$ messages $x_{\CU}$ as the following
\begin{equation}
    \Bx_{\hat{\CK}} = \sum_{\CU \subseteq \hat{\CK}, |\CU| = \hat{t}+1}\Bv_{\CU}x_{\CU}.
\end{equation}
As a result, the received signal at user $k \in \hat{\CK}$ can be written as
\begin{equation} \label{eq:received_signal}
    y_{k} = \sum_{\CU \subseteq \hat{\CK}, \CU \ni k}\Bh_{k}^{H}\underline{\Bv_{\CU}x_{\CU}} + \sum_{\CV \subseteq \hat{\CK} \setminus k, |\CV| = \hat{t}+1}\Bh_{k}^{H}\Bv_{\CV}x_{\CV} + z_k,
\end{equation}
where $z_k$ is the white Gaussian noise. Each of $\binom{\hat{t}+L-1}{\hat{t}}$ underlined terms in~\eqref{eq:received_signal} contains a fresh data  for user $k$ with size $c_k = \frac{\binom{K-\hat{t}-1}{t_k - \hat{t}} }{ \binom{K}{t_k} \binom{t_k}{\hat{t}}  \binom{K-\hat{t}-1}{L - 1}}$, and the rest $\binom{\hat{t}+L-1}{\hat{t+1}}$ terms are seen as interference. Thus, from user $k$ perspective, $y_k$ is a \ac{MAC} with $D = \binom{\hat{t}+L-1}{\hat{t}}$ desired message and $I = \binom{\hat{t}+L-1}{\hat{t}+1}$ interference terms. Let us denote $\CD_k = \{\CU \ | \ \CU \subseteq \hat{\CK}, |\CU| = \hat{t}+1, \CU \ni k\}$ as the set of all the desired message indices for user $k$, i.e., $|\CD_k| = D$. Now, suppose user $k$ can decode all the $D$ desired messages with equal rate as follows\footnote{Symmetric rate is imposed to minimize the overall time to decode all $D$ messages.}
\begin{equation}\label{eq:MAC_rate}
    R^{k}_{\text{MAC}} = \min_{\CQ \subseteq \CD_k, |\CQ| \neq 0} \frac{1}{|\CQ|}R_{\text{sum}}^{\CQ},
\end{equation}
where $R_{\text{sum}}^{\CQ} = \log\left(1 + \frac{\sum_{\CU \in \CQ}|\Bh_{k}^{H}\Bv_{\CU}|^2}{\sum_{\CV \in \CI_k}|\Bh_{k}^{H}\Bv_{\CV}|^2 + \sigma^2}\right)$, and $\CI_k := \{\CV \ | \ \CV \subseteq \hat{\CK} \setminus k, |\CV| = \hat{t}+1\}$ is the set of interfering message indices for user $k$. Since user $k$ receives $D$ messages in each transmission, its overall symmetric rate is equal to $DR^{k}_{\text{MAC}}$. On the other hand, the total size of the received data is equal to $Dc_k$, which requires $T_k = \frac{Dc_k}{DR^{k}_{\text{MAC}}} = \frac{c_k}{R^{k}_{\text{MAC}}}$ seconds. Thus, the required transmission time to serve all the users in $\hat{\CK}$ is equal to $\max_{k \in \hat{\CK}}T_{k}$.

Since we aim to provide a uniform quality of experience throughout the network, the beamformer optimization problem can be then formulated as $\underset{\{\Bv_{\CU}\}}\min \ \underset{k \in \hat{\CK}}\max \ T_{k}$, or equivalently as $\underset{\{\Bv_{\CU}\}}\max \ \underset{k \in \hat{\CK}}\min \ \frac{R^{k}_{\text{MAC}}}{c_k}$. Finally, the weighted rate maximization for a given transmission can be formulated as follows
\begin{equation} 
\begin{array} {l}
	\label{opt:nonconvex_WMMF}
		\underset{\substack{\{\Bv_{\CU}, \gamma^k_{\CU}, R_{\text{sum}}^{\CQ} \}}}{\max}  \underset{k \in \hat{\CK} }{\min} \ \underset{\substack{\CQ \subseteq {\CD_k}, \\ |\CQ| \neq 0}}{\min} \ 
	
        \frac{1}{c_k|\CQ|}R_{\text{sum}}^{\CQ}
	\\
	 \mathrm{subject  \ to} \\ 
       R_{\text{sum}}^{\CQ} \leq \log\left(1 + \sum_{\CU \in \CQ}\gamma^{k}_{\CU}\right), \quad \forall k \in \hat{\CK}, \forall \CQ \subseteq {\CD_k}, |\CQ| \neq 0 \\
     \ds \gamma^{k}_{\CU} \leq \frac{|\Bh_{k}^{H}\Bv_{\CU}|^2}{\sum_{\CV \in \CI_k}|\Bh_{k}^{H}\Bv_{\CV}|^2 + \sigma^2}, \quad \forall k \in \hat{\CK}, \forall \CU \in {\CD}_k,
    \\
	 \ds 
        \sum_{\substack{\CU \subseteq \hat{\CK}, \\ |\CU| = \hat{t}+1}}\|\Bv_{\CU}\|^2\leq P_T,
\end{array}
\end{equation}
where $P_T$ is the total available power at the transmitter. Problem~\eqref{opt:nonconvex_WMMF} can be equivalently rewritten in epigraph form as follows
\begin{subequations}\label{opt:nonconvex_WMMF_epi}
\begin{align}
    \max_{\{\Bv_{\CU}, \gamma^k_{\CU}, R_{k}, R\}} &R \nonumber\\
    \textrm{s.t.} \quad &R \leq \frac{1}{c_k}R_k \, , \quad \forall k \in \hat{\CK} \; , \\
    & R_k \leq \frac{1}{|\CQ|}\log\left(1 + \sum_{\CU \in \CQ}\gamma^{k}_{\CU}\right), \quad \forall k \in \hat{\CK}, \forall \CQ \subseteq {\CD_k}, |\CQ| \neq 0 \; ,   \\ 
    &\gamma^{k}_{\CU} \leq \frac{|\Bh_{k}^{H}\Bv_{\CU}|^2}{\sum_{\CV \in \CI_k}|\Bh_{k}^{H}\Bv_{\CV}|^2 + \sigma^2}, \quad \forall k \in \hat{\CK}, \forall \CU \in {\CD}_k,\label{const:MSE terms} \\
        &\sum_{\substack{\CU \subseteq \hat{\CK}, \\ |\CU| = \hat{t}+1}}\|\Bv_{\CU}\|^2\leq P_T.
\end{align}
\end{subequations}

Note that problem~\eqref{opt:nonconvex_WMMF_epi} is a NP-hard, non-convex problem due to non-convex constraint in~\eqref{const:MSE terms}. However, it can be approximated by an equivalent convex problem using \ac{SCA} method as discussed in details in~\cite{tolli2017multi}. To this end, we first rewrite~\eqref{const:MSE terms} as
\begin{equation}\label{eq:MSE terms}
    \sum_{\CV \in \CI_k}|\Bh_{k}^{H}\Bv_{\CV}|^2 + \sigma^2 \leq \frac{\sum_{\CV \in \CI_k \cup \CU}|\Bh_{k}^{H}\bar{\Bv}_{\CV}|^2 + \sigma^2}{1+{\gamma}^{k}_{\CU}}.
\end{equation}
Now, using the first order Taylor expansion, we can approximate the right hand side of~\eqref{eq:MSE terms} as 
\begin{equation}\label{eq: MSE_approx}
\begin{aligned}
    \mathcal {L}(\mathbf {v}_{\mathcal {V}}, \mathbf {h}_{k}, \gamma _{\mathcal {U}}^{k}) \triangleq & \Big(\sum_{\CV \in \CI_k \cup \CU} \big( 2\mathbb{R}(\bar{\Bv}_{\CV}^H\Bh_{k}\Bh_{k}^{H}\Bv_{\CV}) -|\Bh_{k}^{H}\bar{\Bv}_{\CV}|^2\big)  \\ & \qquad- \frac{\sum_{\CV \in \CI_k \cup \CU}{|\Bh_{k}^{H}\bar{\Bv}_{\CV}|^2 + \sigma^2}}{1+\bar{\gamma}^{k}_{\CU}}({\gamma}^{k}_{\CU}-\bar{\gamma}^{k}_{\CU})+ \sigma^2 \Big) \frac{1}{{1+\bar{\gamma}^{k}_{\CU}}},
\end{aligned}
\end{equation}
where, $\bar{\Bv}_{\CV}$ and $\bar{\gamma}^{k}_{\CU}$ are the fixed approximation points. As a result, substituting~\eqref{eq: MSE_approx} in~\eqref{eq:MSE terms}, problem~\eqref{opt:nonconvex_WMMF_epi} can be approximated as following convex problem
\begin{subequations}\label{opt: convex_WMMF_epi}
\begin{align}
    \max_{\{\Bv_{\CU}, \gamma^k_{\CU}, R_{k}, R\}} &R \nonumber\\
    \textrm{s.t.} \quad &R \leq \frac{1}{c_k}R_k \, , \quad \forall k \in \hat{\CK} \; , \\
    & R_k \leq \frac{1}{|\CQ|}\log\left(1 + \sum_{\CU \in \CQ}\gamma^{k}_{\CU}\right), \quad \forall k \in \hat{\CK}, \forall \CQ \subseteq {\CD_k}, |\CQ| \neq 0 \; ,   \\ 
    &\sum_{\CV \in \CI_k}|\Bh_{k}^{H}\Bv_{\CV}|^2 + \sigma^2 \leq \mathcal {L}(\mathbf {v}_{\mathcal {V}}, \mathbf {h}_{k}, \gamma _{\mathcal {U}}^{k}), \quad \forall k \in \hat{\CK}, \forall \CU \in {\CD}_k,\\
        &\sum_{\substack{\CU \subseteq \hat{\CK}, \\ |\CU| = \hat{t}+1}}\|\Bv_{\CU}\|^2\leq P_T.
\end{align}
\end{subequations}

It is worth mentioning that assuming independent user channels (i.e., $\mathbb{E}\{\Bh_k^H\Bh_{\bar{k}}\} = 0, \forall k \neq \bar{k}$), the solution of~\eqref{opt: convex_WMMF_epi} results in $\frac{R_k}{c_k} = \frac{R_{\bar{k}}}{c_{\bar{k}}}$, i.e., $\frac{R_k}{1-m(s_k)} = \frac{R_{\bar{k}}}{1-m(s_{\bar{k}})}, \forall (k, \bar{k}) \in \hat{\CK}, k \neq \bar{k}$.
\begin{remark} \label{remark: approximated delivery time}
Let us denote $T_{\hat{\CK}} := \max\{\frac{c_k}{R_k}\}, \ \forall k \in \hat{\CK}$, as the transmission time to serve the users in $\hat{\CK}$, where $R_k$ is computed in~\eqref{opt: convex_WMMF_epi}. Then, the total required time to deliver all the messages to all the users can be expressed as $T_T = \sum_{\hat{\CK} \subseteq \CK}T_{\hat{\CK}}$. Now, based on the statement above, at the optimal point, we have $\frac{R_k}{1-m(s_k)} = \frac{R_{\bar{k}}}{1-m(s_{\bar{k}})}, \forall (k, \bar{k}) \in \hat{\CK}, k \neq \bar{k}$. Let us denote $R_{\text{WMM}} := \frac{R_k}{1-m(s_k)}$ as the common weighted rate. As a result, $T_{\hat{\CK}}$ can be expressed as $T_{\hat{\CK}} = \frac{K}{\binom{K}{\hat{t}+L}\binom{\hat{t}+L}{\hat{t}}LR_{\text{WMM}}}$. Note that $T_{\hat{\CK}}$ is independent of the users' states and is equal for all $k \in \hat{\CK}$. Now, assuming $R_{\text{WMM}}$ is almost the same for any group of targeted users $\hat{\CK}$, we can Approximate $T_T$ as $T_{\hat{\CK}} = \frac{K}{\binom{\hat{t}+L}{\hat{t}}LR_{\text{WMM}}}$. Consequently, defining $R^{\text{sym}}_{\text{WMM}}$ as $R^{\text{sym}}_{\text{WMM}} := \frac{K}{T_T}$ results in $R^{\text{sym}}_{\text{WMM}} = \binom{\hat{t}+L}{\hat{t}}LR_{\text{WMM}}$. Following similar arguments, we can express $R^{\text{sym}}_{\text{MM}} = \binom{{t}+L}{{t}}LR_{\text{MM}}$ as the symmetric rate for uniform memory loading case proposed in~\cite{tolli2017multi}, where $t = \frac{KM}{S}$, $R_{\text{MM}} = \frac{\bar{R}_k}{1-{M}/{S}}$, and $\bar{R}_k$ is the common max-min rate for the symmetric cache placement case in~\cite{tolli2017multi}.
\end{remark}

Based on remark~\ref{remark: approximated delivery time}, there exist a trade-off between the rate improvement due to the weighted-max-min formulation and the \emph{global caching gain} as the following
\begin{equation}
    \frac{R^{\text{sym}}_{\text{WMM}}}{R^{\text{sym}}_{\text{MM}}} = \frac{\binom{\hat{t}+L}{\hat{t}}R_{\text{WMM}}}{\binom{{t}+L}{{t}}R_{\text{MM}}}.
\end{equation}
In other words, when compared with symmetric cache placement in~\cite{tolli2017multi}), we can improve the delivery time if the DoF loss (i.e., $\frac{\binom{\hat{t}+L}{\hat{t}}}{\binom{{t}+L}{{t}}} \leq 1$) is negligible compared to the multi-rate gain (i.e., $\frac{R^{\text{sym}}_{\text{WMM}}}{R^{\text{sym}}_{\text{MM}}} \geq 1$). In simulation results, we will discuss different scenarios in which we have a significant multi-rate gain that is much larger than one.

\begin{remark} 
The proposed delivery scheme is based on the minimum available cache ratio of users located in different states. As a result, the performance may be limited due to min operation for some cases where there exist a limited number of users with low available cache against a much larger number of users with notably higher available memory. For example, for the case $\Bt = \{4,3,3,3,0\}$, the proposed method will be limited to $\hat{t} = 0$, which is basically the traditional unicasting. However, assuming user $5$ is located in some location with $t(s_5) > 3$, will increase the common cache ratio by $3$, which will improve the delivery. A detailed discussion on this idea is provided in section~\ref{Sec:phantom user}.
\end{remark}
